SWIFT: Rapid Decentralized Federated Learning via Wait-Free Model Communication

The decentralized Federated Learning (FL) setting avoids the role of a potentially unreliable or untrustworthy central host by utilizing groups of clients to collaboratively train a model via localized training and model/gradient sharing. Most existing decentralized FL algorithms require synchronization of client models where the speed of synchronization depends upon the slowest client. In this work, we propose SWIFT: a novel wait-free decentralized FL algorithm that allows clients to conduct training at their own speed. Theoretically, we prove that SWIFT matches the gold-standard iteration convergence rate $\mathcal{O}(1/\sqrt{T})$ of parallel stochastic gradient descent for convex and non-convex smooth optimization (total iterations $T$). Furthermore, we provide theoretical results for IID and non-IID settings without any bounded-delay assumption for slow clients which is required by other asynchronous decentralized FL algorithms. Although SWIFT achieves the same iteration convergence rate with respect to $T$ as other state-of-the-art (SOTA) parallel stochastic algorithms, it converges faster with respect to run-time due to its wait-free structure. Our experimental results demonstrate that SWIFT's run-time is reduced due to a large reduction in communication time per epoch, which falls by an order of magnitude compared to synchronous counterparts. Furthermore, SWIFT produces loss levels for image classification, over IID and non-IID data settings, upwards of 50% faster than existing SOTA algorithms.

==> Baseline-Time.tex <==
\begin{table}[!htbp]
    \centering
    \setlength\extrarowheight{2pt}
    \resizebox{0.75\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        Decentralized FL &\multicolumn{4}{c|}{16 Client Ring} \\ 
        \cline{2-5} Algorithms & Epoch (s) & \% Change & Comm. (s) & \% Change \\
        \hline
        \textbf{\ouralgo} ($I_1 = 0$) & \textbf{1.019} & --- & \textbf{0.086} & --- \\
        D-SGD ($I_1 = 0$) & 1.558 & +52.89 & 0.627 & +646.43 \\
        \hline
        \textbf{\ouralgo} ($I_1 = 1$) & \textbf{1.016} & -0.29&\textbf{0.064} & -23.81\\
        LD-SGD ($I_1 = 1$) & 1.320 & +29.54 & 0.428 & +409.52 \\
        PA-SGD ($I_1 = 1$) & 1.281 & +25.71 & 0.358 & +326.19 \\
        \hline
    \end{tabular}
    }
    \caption{Average epoch and communication times on CIFAR-10 for 16 client ring.}
    \label{tab:baseline}
\end{table}
